Towards Unified Benchmark and Models for Multi-Modal Perceptual Metrics

Human perception of similarity across uni- and multimodal inputs is highly complex, making it challenging to develop automated metrics that accurately mimic it. General purpose vision-language models, such as CLIP and large multi-modal models (LMMs), can be applied as zero-shot perceptual metrics, and several recent works have developed models specialized in narrow perceptual tasks. However, the extent to which existing perceptual metrics align with human perception remains unclear. To investigate this question, we introduce UniSim-Bench, a benchmark encompassing 7 multi-modal perceptual similarity tasks, with a total of 25 datasets. Our evaluation reveals that while general-purpose models perform reasonably well on average, they often lag behind specialized models on individual tasks. Conversely, metrics fine-tuned for specific tasks fail to generalize well to unseen, though related, tasks. As a first step towards a unified multi-task perceptual similarity metric, we fine-tune both encoder-based and generative vision-language models on a subset of the UniSim-Bench tasks. This approach yields the highest average performance, and in some cases, even surpasses taskspecific models. Nevertheless, these models still struggle with generalization to unseen tasks, highlighting the ongoing challenge of learning a robust, unified perceptual similarity metric capable of capturing the human notion of similarity. The code and models are available at https://github.com/SaraGhazanfari/UniSim.

==> arxiv <==
@String(PAMI = {IEEE Trans. Pattern Anal. Mach. Intell.})
@String(IJCV = {Int. J. Comput. Vis.})
@String(CVPR= {IEEE Conf. Comput. Vis. Pattern Recog.})
@String(ICCV= {Int. Conf. Comput. Vis.})
@String(ECCV= {Eur. Conf. Comput. Vis.})
@String(NIPS= {Adv. Neural Inform. Process. Syst.})
@String(ICPR = {Int. Conf. Pattern Recog.})
@String(BMVC= {Brit. Mach. Vis. Conf.})
@String(TOG= {ACM Trans. Graph.})
@String(TIP  = {IEEE Trans. Image Process.})
@String(TVCG  = {IEEE Trans. Vis. Comput. Graph.})
@String(TMM  = {IEEE Trans. Multimedia})
@String(ACMMM= {ACM Int. Conf. Multimedia})
@String(ICME = {Int. Conf. Multimedia and Expo})
@String(ICASSP=	{ICASSP})
@String(ICIP = {IEEE Int. Conf. Image Process.})
@String(ACCV  = {ACCV})
@String(ICLR = {Int. Conf. Learn. Represent.})
@String(IJCAI = {IJCAI})
@String(PR   = {Pattern Recognition})
@String(AAAI = {AAAI})
@String(CVPRW= {IEEE Conf. Comput. Vis. Pattern Recog. Worksh.})
@String(CSVT = {IEEE Trans. Circuit Syst. Video Technol.})

@String(SPL	= {IEEE Sign. Process. Letters})
@String(VR   = {Vis. Res.})
@String(JOV	 = {J. Vis.})
@String(TVC  = {The Vis. Comput.})
@String(JCST  = {J. Comput. Sci. Tech.})
@String(CGF  = {Comput. Graph. Forum})
@String(CVM = {Computational Visual Media})


@String(PAMI  = {IEEE TPAMI})
@String(IJCV  = {IJCV})
@String(CVPR  = {CVPR})
@String(ICCV  = {ICCV})
@String(ECCV  = {ECCV})
@String(NIPS  = {NeurIPS})
@String(ICPR  = {ICPR})
@String(BMVC  =	{BMVC})
@String(TOG   = {ACM TOG})
@String(TIP   = {IEEE TIP})
@String(TVCG  = {IEEE TVCG})
@String(TCSVT = {IEEE TCSVT})
@String(TMM   =	{IEEE TMM})
@String(ACMMM = {ACM MM})
@String(ICME  =	{ICME})
@String(ICASSP=	{ICASSP})
@String(ICIP  = {ICIP})
@String(ACCV  = {ACCV})
@String(ICLR  = {ICLR})
@String(IJCAI = {IJCAI})
@String(PR = {PR})
@String(AAAI = {AAAI})
@String(CVPRW= {CVPRW})
@String(CSVT = {IEEE TCSVT})



@misc{Authors14,
 author = {FirstName LastName},
 title = {The frobnicatable foo filter},
 note = {Face and Gesture submission ID 324. Supplied as supplemental material {\tt fg324.pdf}},
 year = 2014
}

@misc{Authors14b,
 author = {FirstName LastName},
 title = {Frobnication tutorial},
 note = {Supplied as supplemental material {\tt tr.pdf}},
 year = 2014
}

@article{Alpher02,
author = {FirstName Alpher},
title = {Frobnication},
journal = PAMI,
volume = 12,
number = 1,
pages = {234--778},
year = 2002
}

@article{Alpher03,
author = {FirstName Alpher and  FirstName Fotheringham-Smythe},
title = {Frobnication revisited},
journal = {Journal of Foo},
volume = 13,
number = 1,
pages = {234--778},
year = 2003
}

@article{Alpher04,
author = {FirstName Alpher and FirstName Fotheringham-Smythe and FirstName Gamow},
title = {Can a machine frobnicate?},
journal = {Journal of Foo},
volume = 14,
number = 1,
pages = {234--778},
year = 2004
}

@inproceedings{Alpher05,
author = {FirstName Alpher and FirstName Gamow},
title = {Can a computer frobnicate?},
booktitle = CVPR,
pages = {234--778},
year = 2005
}


==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/0_abstract.tex <==
\begin{abstract}

\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}


==> sec/2_related_works.tex <==
\section{Related Works}
\label{sec:related_work}




\paragraph{Perceptual Similarity Metric.}
(2AFC
3AFC)

\begin{itemize}
    \item LPIPS
    \item DreamSim
    \item robust versions, LipSim, RobustCLIP
\end{itemize}


\paragraph{Multimodal Similarity Metric.} (IQA
perc. attributes
text-images-FC
text 2AFC)
\begin{itemize}
    \item Exploring CLIP for Assessing the Look and Feel of Images
    \item VIEScore: Towards Explainable Metrics for Conditional Image Synthesis Evaluation (not sure about this because it's about explainability)
    \item Human Preference Score: Better Aligning Text-to-Image Models with Human Preference 
    \item Descriptive Image Quality Assessment in the Wild
    \item InfoMetIC: An Informative Metric for Reference-free Image Caption Evaluation
    \item UMIC: An Unreferenced Metric for Image Captioning via Contrastive Learning
    \item Human Preference Score v2: A Solid Benchmark for Evaluating Human Preferences of Text-to-Image Synthesis
    \item Polos: Multimodal Metric Learning from Human Feedback for Image Captioning (reference-with-image, different from our setting)
    \item Positive-Augmented Contrastive Learning for Image and Video Captioning Evaluation (most recent reference-free)
\end{itemize}  

\paragraph{Large Multi-modal Models.}
In this paragraph we have both general multi-image model and those which are trained for perceptual tasks
\textbf{In general}:

\begin{itemize}
    \item MANTIS: Interleaved Multi-Image Instruction Tuning
    \item LLaVA-NeXT-Interleave: Tackling Multi-image, Video, and 3D in Large Multimodal Models
    \item mPLUG-Owl3: Towards Long Image-Sequence Understanding in Multi-Modal Large Language Models
\end{itemize}

\textbf{Trained for Image quality assessment}:

\begin{itemize} 
    \item 2AFC Prompting of Large Multimodal Models for Image Quality Assessment
    \item Large Multi-modality Model Assisted AI-Generated Image Quality Assessment
    \item Adaptive Image Quality Assessment via Teaching Large Multimodal Model to Compare
    \item AesExpert: Towards Multi-modality Foundation Model for Image Aesthetics Perception
    \item Co-instruct Towards Open-ended Visual Quality Comparison: mplug-OWL2 --- not multi-image
\end{itemize}

\paragraph{Benchmarks.}

\begin{itemize}
    \item BLINK: Multimodal Large Language Models Can See but Not Perceive 
    \item Holistic Evaluation of Text-To-Image Models 
    \item MuirBench: A Comprehensive Benchmark for Robust Multi-image Understanding
    \item ImagenHub: Standardizing the evaluation of conditional image generation models
    \item AIGIQA-20K: A Large Database for AI-Generated Image Quality Assessment
    \item AGIQA-3K: An Open Database for AI-Generated Image Quality Assessment
    \item A-Bench: Are LMMs Masters at Evaluating AI-generated Images?
    \item  Q-Bench: A benchmark for general-purpose foundation models on low-level vision
    \item Q-BENCH+: A Benchmark for Multi-modal Foundation Models on Low-level Vision from Single Images to Pairs
    \item MIBench: Evaluating Multimodal Large Language Models over Multiple Images
\end{itemize}    

\paragraph{Training Data}

\begin{itemize}
    \item Pick-a-Pic: An Open Dataset of User Preferences for Text-to-Image Generation 
    \item Human Preference Score: Better Aligning Text-to-Image Models with Human Preference 
    \item Validated Image Caption Rating Dataset
\end{itemize}















==> sec/3_method.tex <==
\section{Method}
\label{sec:method}


==> sec/4_experiments.tex <==
\section{Experiments}
\label{section:exp}
